MVEB: Self-Supervised Learning with Multi-View Entropy Bottleneck

Self-supervised learning aims to learn representation that can be effectively generalized to downstream tasks. Many self-supervised approaches regard two views of an image as both the input and the self-supervised signals, assuming that either view contains the same task-relevant information and the shared information is (approximately) sufficient for predicting downstream tasks. Recent studies show that discarding superfluous information not shared between the views can improve generalization. Hence, the ideal representation is sufficient for downstream tasks and contains minimal superfluous information, termed minimal sufficient representation. One can learn this representation by maximizing the mutual information between the representation and the supervised view while eliminating superfluous information. Nevertheless, the computation of mutual information is notoriously intractable. In this work, we propose an objective termed multi-view entropy bottleneck (MVEB) to learn minimal sufficient representation effectively. MVEB simplifies the minimal sufficient learning to maximizing both the agreement between the embeddings of two views and the differential entropy of the embedding distribution. Our experiments confirm that MVEB significantly improves performance. For example, it achieves top-1 accuracy of 76.9\% on ImageNet with a vanilla ResNet-50 backbone on linear evaluation. To the best of our knowledge, this is the new state-of-the-art result with ResNet-50.

==> doc/answers.tex <==
{
\onecolumn
%\normalsize

\noindent\textbf{Responses to the Reviewers and Editor}

\section*{\textbf{Reviewer 1}}


\ \\


\begin{myblock}{Comment 1-1}
The clarification on MVIB and MVEB differentiation is enlightening. The authors should highlight this distinction more prominently in their main text to avoid potential misunderstandings. The additional ablation experiments and the intent to release their code and models add substantial value.

\end{myblock}

\textbf{Response:}
Thank you for your constructive suggestion.
We highlight this distinction in Section \ref{sec:MVEB} in the revised manuscript.

\ \\

\begin{myblock}{Comment 1-2}
This new addition substantially solidifies MVEB's standing as a competent and efficient framework. It would be beneficial to include more specific details of this study in the main text to further quantify this efficiency advantage.
\end{myblock}
\textbf{Response:}
Thank you for your suggestion. We add more specific details of the pretraining efficiency study in Section \ref{PE} in the revised manuscript.
\ \\

\begin{myblock}{Comment 1-3}
This expansion is a positive development, but the authors might consider testing even more architectures or settings in the future to fortify the claim of MVEB's generalizability.

\end{myblock}
\textbf{Response:} 
Our limited GPU resources and the constrained timeline for the rebuttal prevent us from testing many architectures or settings. In this new version, we add more results of MVEB on Resnet18 and Resent34 in Table \ref{tab:mask}. 

\ \\
\begin{myblock}{Comment 1-4}
Additionally, there are still some typos and logical issues in the revised manuscript. For example:

On page 6, the last part of Sec 4, the equation number "Eq. (??)" seems like a placeholder and should be replaced with the appropriate equation number for clarity.

Therefore, I would suggest the authors conduct a more thorough proof-read of the words and logic of this submission.
\end{myblock}

\textbf{Response:}
Thanks for the correction. We have conducted a  thorough proof-read of the words and logic of the new submission.



% {
% \onecolumn
% %\normalsize

% \noindent\textbf{Responses to the Reviewers and Editor}

% \section*{\textbf{Reviewer 1}}


% \ \\


% \begin{myblock}{Comment 1-1}
%  Time complexity analysis is encouraged to be added. Is the newly designed objective easy to be computed?
% \end{myblock}

% \textbf{Response:}
% Thanks for the comments. We assume the batch-size is $n$ and the dimensionality of the output of the Siamese network is $d$. Time complexity analysis is O($(d+n+2)n^2$).
% The newly designed objective is easy to be computed. MVEB can be directly applied to the Siamese network without modification of the network. In Section \ref{PE}, we conduct the study of pretraining efficiency. The pretraining cost of MVEB is less than BYOL and Barlow Twins.


% \ \\

% \begin{myblock}{Comment 1-2}
% It seems some strong and important baselines are missing. For example, those masked autoencoder-based methods including MAE, SimMM.
% \end{myblock}
% \textbf{Response:}
% We compare our method with the masked autoencoder-based methods for linear evaluation on ImageNet. As shown in Table \ref{tab:mask}, MVEB outperforms MAE and SimMM.


% \ \\

% \begin{myblock}{Comment 1-3}
% Equation 7 seems incorrect. The first term of the $L_vMVIB$. It should be $P(z1|v1)||p(z2|v2)$ instead.
% \end{myblock}
% \textbf{Response:}
% Thanks for the correction. We have fixed this typo in
% the revised manuscript.
% \ \\

% \begin{myblock}{Comment 1-4}
% The motivation of defining $q_{\theta}(z_1|v_2)$ as the von Mises-Fisher(vMF) distribution is unclear.
% \end{myblock}
% \textbf{Response:}
% For self-supervised learning based on the Siamese network, such as SimCLR, BYOL, and SimSiam,  the representation $\mathbf{z_1}$ is $\ell_2$-normalized in the hypersphere space to improve the performance of the models. We also normalize $\mathbf{z_1}$ in  the hypersphere space. The von Mises-Fisher (vMF) is  the common distribution  of the hypersphere space. Hence, we define $q_{\phi}(\mathbf{z_1}|\mathbf{v_2})$ as the vMF  distribution, which is similar to the Gaussian distribution in the Euclidean space. We clarified the motivation in the revised manuscript.

% \section*{\textbf{Reviewer 2}}

% \ \\

% \begin{myblock}{Comment 2-1}
%  I have a basic doubt about the premise of the algorithm that the SSL representation only needs to learn the necessary information and that can be found by finding the synergies between the augmented views. Here is a practical scenario I can think of -- suppose the two augmentations are "RandomHorizontalFlip" and "RandomGrayscale". Here, the common information between these two augmented views will be the shape of the object in general and the information about "color" should be discarded as it is only present in one image. The same representation, now if used for a downstream task which is about classifying color vs black-and-white images, may not work optimally because the representation has learned to ignore the color information during training. I would like the authors to provide more justification regarding the notion of explicitly discarding superfluous information from augmented views and how it can mitigate a scenario I mentioned.
% \end{myblock}

% \textbf{Response:}
% Thanks for the comments. It is a very valuable comment. As described in
% Section \ref{ss:dc}, we discuss this general problem for the limitation of MVEB. Explicitly discarding superfluous information from augmented views is based on the assumption in multi-view learning: either view is (approximately) sufficient for the prediction of downstream tasks and contains the same task-relevant information.  The practical scenario presented by the reviewer violates this assumption. However, this is the key problem for existing self-supervised learning methods based on view augmentations. 
% The paper "What Should not be contrastive in contrastive learning, ICLR 2021" proposes the leave-one-out alignment to solve this problem. This method is also applied to our framework to solve the problem of the  scenario the reviewer mentioned. 



% \ \\

% \begin{myblock}{Comment 2-2}
% Authors should consider providing more information (or proof) regarding the decompositions mentioned in Eq.8 and Eq. 9. Are these based on intuitions only?
% \end{myblock}
% \textbf{Response:}
% Thanks very much for the comments. The proofs of $I_\phi\left(\mathbf{z_1} ; \mathbf{v_1} |\mathbf{v_2}\right)=H(\mathbf{z_1}|\mathbf{v_2})-H(\mathbf{z_1}| \mathbf{v_1},\mathbf{v_2})$ and $I_\phi\left(\mathbf{z_1} ; \mathbf{v_1} \right)=H(\mathbf{z_1})-H(\mathbf{z_1}| \mathbf{v_1})$ have been added to the appendix
% of the revised manuscript.


% \ \\

% \begin{myblock}{Comment 2-3}
% The background on Stein's estimator can potentially be part of supplementary materials.
% \end{myblock}
% \textbf{Response:}
% We have put this part in the appendix.

% \section*{\textbf{Reviewer 3}}

% \ \\

% \begin{myblock}{Comment 3-1}

% This work is developed based on several prior works within the area. The main contribution is the MVEB framework which relaxes some constraints of MVIB to reach better performance and efficiency. The design logic is clear and complete but a bit lacking novelty. The comparative study is as comprehensive as prior works and the superiority of MVEB seems overt, which is regarded as the main contribution of this work. However, the ablation study is rather limited. More analysis and details on the design receipt should be supplemented to further enhance novelty. Moreover, the authors are recommended making the proposed model publicly accessible to enable future development.
% \end{myblock}
% \textbf{Response:}
% Thank you very much for the comments. 

% \textbf{Novelty} \textbf{(1).}  We don't  relax some constraints of MVIB. 
% MVIB cannot be directly applied to the Siamese network due to the intractability of the computation of mutual information. 
% As mentioned in Section \ref{ss:MVIB}, the variational method  can be introduced to optimize MVIB. However, 
% this approximation optimization requires additional stochastic networks and does not work as expected in practice for visual recognition models. We derive the novel MVEB framework to solve the challenge of learning the  minimal sufficient representation, which includes the new entropy target (Eq. (\ref{mvebsss})),  the new approximation optimation conditional entropy $H(\mathbf{z_1}|\mathbf{v_2})$,  the analysis of the approximation optimation for $H(\mathbf{z_1}|\mathbf{v_2})$ to guarantee to achieve the minimization of $H(\mathbf{z_1}|\mathbf{v_2})$, and  the  score-based entropy estimator with the
% von Mises-Fisher kernel to approximate the gradient of $H(\mathbf{z_1})$. 

%  \textbf{Novelty} \textbf{(2)}.  We first analyze contrastive learning (e.g., SimCLR and MOCO), asymmetric network methods (e.g., BYOL and SimSiam), and feature decorrelation methods (e.g., Barlow Twins and  VICReg) from learning the  minimal sufficient representation in Section \ref{RAU}. Based on MVEB, we argue that these methods also try to learn the minimal sufficient representation by optimizing  alignment and uniformity.

% \textbf{Ablation Expreiments}. 
% We now add three ablation experiments to validate the effectiveness of the design of MVEB
% which are the comparison of MVEB with MVIB, generalization across different backbones, and pretraining efficiency. MVEB is theoretically
%  derived as the optimization objective, which can directly be applied to the Siamese network without  modification of the network.

% If our paper is accepted, we will release the code and the pre-trained models of MVEB.

% \ \\

% \begin{myblock}{Comment 3-2}
%  The authors mentioned several times the problem related to the efficiency of previous frameworks, i.e., “the computation of the mutual information is notoriously intractable”. MVEB, however, is claimed to be directly applied to the Siamese network without modification of the network structure and other complex designs. In the experiments, the authors mainly compare the performance while a shred of evidence on efficiency is missing. Therefore, the authors are recommended to conduct such a study to validate their claim.
% \end{myblock}

% \textbf{Response:}
% Thanks for the comments.  In Section \ref{PE}, we add a new study of pretraining efficiency. The pretraining cost of MVEB is less than BYOL and Barlow Twins.





% \ \\

% \begin{myblock}{Comment 3-3}
% In the experiments, only MVEB with the ResNet-50 backbone is tested. More variances on different backbone networks are recommended to be supplemented to further demonstrate generalizability.
% \end{myblock}
% \textbf{Response:}
%  We add a new comparison on Vison Transformer in Table \ref{tab:dfb}. The result of MVEB on Rresnet101 is provided in Table \ref{tab:mask}. 
% \ \\

% \begin{myblock}{Comment 3-4}
% This work seems thorough and comprehensive. The proposed method is novel in the sense that it provides a new perspective on the targeted task. The experiments show that the proposed method is achieving promising results on standard benchmarks. However, since I am not directly working on this topic, I leave more room for other reviewers in making the final decision.
% \end{myblock}
% \textbf{Response:}
%  Thank you very much for your support.





==> doc/cover.tex <==
{{
\twocolumn[
\begin{@twocolumnfalse}
\thispagestyle{empty}


\noindent
Dear Editor-in-Chief, Associate Editor, and Reviewers,

\ \\
Thank you very much for reviewing our submission and providing your valuable comments.

\ \\
We have revised this version by addressing the reviewers' comments and incorporating their suggestions.
All the changes in the current version are highlighted in \wenljx{blue}.
Detailed responses to the reviewers' comments are put at the end of this manuscript.
%Detailed responses to reviewers' comments are appended at the end of this manuscript.

\ \\
Thank you very much.

\ \\
Sincerely,\\ \\
\noindent
Liangjian Wen

\end{@twocolumnfalse}
]
\clearpage
%\setcounter{page}{1}
}}
